A flexible framework for early power and timing comparison of time-multiplexed CGRA kernel executions

At the intersection between traditional CPU architectures and more specialized options such as FPGAs or ASICs lies the family of reconfigurable hardware architectures, termed Coarse-Grained Reconfigurable Arrays (CGRAs). CGRAs are composed of a 2-dimensional array of processing elements (PE), tightly integrated with each other, each capable of performing arithmetic and logic operations. The vast design space of CGRA implementations poses a challenge, which calls for fast exploration tools to prune it in advance of time-consuming syntheses. The proposed tool aims to simplify this process by simulating kernel execution and providing a characterization framework. The estimator returns energy and latency values otherwise only available through a time-consuming post-synthesis simulation, allowing for instantaneous comparative analysis between different kernels and hardware configurations.

==> tables/area_breakdown.tex <==
\begin{table}[tp]
\caption{Post-synthesis area breakdown of a $4\times{}4$ CGRA instance. Total area is \SI{\sim 0.4}{\milli\metre\squared} in 65nm technology.}
\vspace{-0.2cm}
\label{tbl:area_breakdown}
\centering
\begin{tabular}{|@{\hskip0.1cm}l@{\hskip0.1cm}||@{\hskip0.1cm}c@{\hskip0.1cm}|@{\hskip0.1cm}c@{\hskip0.1cm}|@{\hskip0.1cm}c@{\hskip0.1cm}|@{\hskip0.1cm}c@{\hskip0.1cm}|@{\hskip0.1cm}c@{\hskip0.1cm}|@{\hskip0.1cm}c@{\hskip0.1cm}|@{\hskip0.1cm}c@{\hskip0.1cm}|}
\hline
Block & 
\begin{tabular}{@{}c@{}}Ctx \& \\ kernel\end{tabular} & 
Sync. &
Ctrl. &
DMA &
\begin{tabular}{@{}c@{}}Program \\ mem.\end{tabular} &
\begin{tabular}{@{}c@{}}ALU \& \\ Muxes\end{tabular} &
\begin{tabular}{@{}c@{}}Data \\ regs.\end{tabular} \\
\hline
Area (\%) & 7  & 4   & 1   & 2 & 39 & 43  & 4 \\
\hline
\end{tabular}
\vspace{-0.2cm}
\end{table}
